Bad Characters: Imperceptible NLP Attacks

Several years of research have shown that machine-learning systems are vulnerable to adversarial examples, both in theory and in practice. Until now, such attacks have primarily targeted visual models, exploiting the gap between human and machine perception. Although text-based models have also been attacked with adversarial examples, such attacks struggled to preserve semantic meaning and indistinguishability. In this paper, we explore a large class of adversarial examples that can be used to attack text-based models in a black-box setting without making any human-perceptible visual modification to inputs. We use encoding-specific perturbations that are imperceptible to the human eye to manipulate the outputs of a wide range of Natural Language Processing (NLP) systems from neural machine-translation pipelines to web search engines. We find that with a single imperceptible encoding injection -- representing one invisible character, homoglyph, reordering, or deletion -- an attacker can significantly reduce the performance of vulnerable models, and with three injections most models can be functionally broken. Our attacks work against currently-deployed commercial systems, including those produced by Microsoft and Google, in addition to open source models published by Facebook, IBM, and HuggingFace. This novel series of attacks presents a significant threat to many language processing systems: an attacker can affect systems in a targeted manner without any assumptions about the underlying model. We conclude that text-based NLP systems require careful input sanitization, just like conventional applications, and that given such systems are now being deployed rapidly at scale, the urgent attention of architects and operators is required.

==> figures/infos/overallpipeline.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{figures/infos/overall_pipeline.pdf}
    \caption{Typical text visualization and NLP processing pipelines, the gap between which is the basis for imperceptible perturbation adversarial examples.}
    \label{fig:overall_pipeline}
\end{figure*}

==> figures/revision/terminal.tex <==
\begin{figure*}[b]
  \centering
  \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/revision/test.png}
    \caption{Screenshot provided by reviewers.}
    \label{fig:reviewer_screenshot}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/revision/terminal.png}
    \caption{Repeated output on MacOS terminal.}
    \label{fig:macos_screenshot}
  \end{minipage}
    \hfill
  \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=.75\linewidth]{figures/revision/difference.png}
    \caption{Pixel-wise string difference on MacOS.}
    \label{fig:terminal_difference}
  \end{minipage}
\end{figure*}

==> tables/bidi_table.tex <==
\begin{table*}[h]
\centering
\begin{adjustbox}{scale=1.0,center}
\begin{tabular}{ll|l}
\toprule
Rendering & Encoded Order & Encoding \\
\midrule
1234 & 1234 & 1 2 3 4 \\
1234 & 1243 & 1 2 {\color{red} U+202B} 4 {\color{blue} U+2067} 3 \\
1234 & 1324 & 1 {\color{blue} U+2067} 3 {\color{green} U+2068} 2 {\color{pink} U+2029} 4 \\
1234 & 1342 & 1 {\color{red} U+202B} 3 {\color{blue} U+2067} 4 2 \\
1234 & 1423 & 1 {\color{red} U+202B} 4 2 {\color{blue} U+2067} 3 \\
1234 & 1432 & 1 {\color{red} U+202B} 4 {\color{blue} U+2067} 3 {\color{green} U+2068} 2 \\
1234 & 2134 & {\color{red} U+202B} 2 {\color{blue} U+2067} 1 {\color{pink} U+2029} 3 4 \\
1234 & 2143 & {\color{red} U+202B} 2 {\color{lime} U+2066}  1 {\color{pink} U+2029} {\color{red} U+202B} 4 {\color{lime} U+2066}  3 \\
1234 & 2314 & {\color{red} U+202B} 2 {\color{blue} U+2067} 3 {\color{yellow} U+2060} 1 {\color{pink} U+2029} 4 \\
1234 & 2341 & {\color{red} U+202B} 2 {\color{blue} U+2067} 3 4 1 \\
1234 & 2431 & {\color{red} U+202B} 2 {\color{green} U+2068} 4 {\color{red} U+202B} 3 {\color{magenta} U+2028} 1 \\
1234 & 3124 & {\color{red} U+202B} 3 1 {\color{blue} U+2067} 2 {\color{pink} U+2029} 4 \\
1234 & 3214 & {\color{red} U+202B} 3 {\color{blue} U+2067} 2 {\color{green} U+2068} 1 {\color{pink} U+2029} 4 \\
1234 & 3241 & {\color{orange} U+202E} 3 {\color{orange} U+202E} 2 4 {\color{brown} U+202C} {\color{brown} U+202C} 1\\
1234 & 3412 & {\color{red} U+202B} 3 4 {\color{blue} U+2067} 1 2\\
1234 & 3421 & {\color{red} U+202B} 3 {\color{blue} U+2067} 4 {\color{green} U+2068} 2 1 \\
1234 & 4123 & {\color{red} U+202B} 4 1 2 {\color{blue} U+2067} 3 \\
1234 & 4132 & {\color{orange} U+202E} {\color{purple} U+202D} 4 {\color{orange} U+202E} 1 3 {\color{brown} U+202C} {\color{brown} U+202C} 2 {\color{brown} U+202C} \\
1234 & 4231 & {\color{red} U+202B} 4 {\color{blue} U+2067} 2 3 {\color{green} U+2068} 1 \\
1234 & 4213 & {\color{orange} U+202E} {\color{purple} U+202D} {\color{orange} U+202E} 4 2 {\color{brown} U+202C} 1 {\color{brown} U+202C} 3 {\color{brown} U+202C} \\
1234 & 4312 & {\color{red} U+202B} 4 3 {\color{blue} U+2067} 1 {\color{green} U+2068} 2 \\
1234 & 4321 & {\color{red} U+202B} 4 {\color{magenta} U+2028} 3 {\color{magenta} U+2028} 2 {\color{magenta} U+2028} 1 \\
\bottomrule
\\
\end{tabular}
\end{adjustbox}
\caption{Reordering through Bidi Algorithm manipulation in Google Chrome on MacOS. Although some are correct and behave according to the specification, quite a few are malformed and should not be rendered. Nevertheless, Google Chrome renders them, allowing for adversarial manipulation.}
\label{tab:bidi-digits}
\end{table*}


==> tables/ling_fam.tex <==
\begin{table}[t]
\centering
\caption{Text mixing {\color{red} Latin} and {\color{blue} Cyrillic} linguistic families.} 
\begin{tabular}{@{}cc@{}}
\toprule
Interword Mixing & Intraword Mixing \\ \midrule
\color{red}{Hello} \color{blue}{\cyrillicp\cyrillica\cyrillicp\cyrillica}       &   \color{red}{Hello} \color{blue}{\cyrillicp}\color{red}{a}\color{blue}{\cyrillicp}\color{red}{a}       \\ \bottomrule
\end{tabular}
\label{tab:lingfam}
\end{table}
